Custom Execution Environments with Containers in Pegasus-enabled Scientific Workflows

Science reproducibility is a cornerstone feature in scientific workflows. In most cases, this has been implemented as a way to exactly reproduce the computational steps taken to reach the final results. While these steps are often completely described, including the input parameters, datasets, and codes, the environment in which these steps are executed is only described at a higher level with endpoints and operating system name and versions. Though this may be sufficient for reproducibility in the short term, systems evolve and are replaced over time, breaking the underlying workflow reproducibility. A natural solution to this problem is containers, as they are well defined, have a lifetime independent of the underlying system, and can be user-controlled so that they can provide custom environments if needed. This paper highlights some unique challenges that may arise when using containers in distributed scientific workflows. Further, this paper explores how the Pegasus Workflow Management System implements container support to address such challenges.

==> plots/storage_skylake/docker_network_usage_master.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3772.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1210,704){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(1210,1111){\makebox(0,0)[r]{\strut{}$20000$}}%
      \put(1210,1517){\makebox(0,0)[r]{\strut{}$40000$}}%
      \put(1210,1924){\makebox(0,0)[r]{\strut{}$60000$}}%
      \put(1210,2331){\makebox(0,0)[r]{\strut{}$80000$}}%
      \put(1210,2738){\makebox(0,0)[r]{\strut{}$100000$}}%
      \put(1210,3144){\makebox(0,0)[r]{\strut{}$120000$}}%
      \put(1210,3551){\makebox(0,0)[r]{\strut{}$140000$}}%
      \put(1342,484){\makebox(0,0){\strut{}$0$}}%
      \put(1814,484){\makebox(0,0){\strut{}$100$}}%
      \put(2285,484){\makebox(0,0){\strut{}$200$}}%
      \put(2757,484){\makebox(0,0){\strut{}$300$}}%
      \put(3228,484){\makebox(0,0){\strut{}$400$}}%
      \put(3700,484){\makebox(0,0){\strut{}$500$}}%
      \put(4171,484){\makebox(0,0){\strut{}$600$}}%
      \put(4643,484){\makebox(0,0){\strut{}$700$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,2127){\rotatebox{-270}{\makebox(0,0){\strut{}Kilobytes/Second}}}%
      \put(2992,154){\makebox(0,0){\strut{}Runtime (Seconds)}}%
      \csname LTb\endcsname%%
      \put(3656,3378){\makebox(0,0)[r]{\strut{}Cluster Size 1}}%
      \csname LTb\endcsname%%
      \put(3656,3158){\makebox(0,0)[r]{\strut{}Cluster Size 12}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plots/storage_skylake/docker_network_usage_master}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/storage_skylake/docker_network_usage_master_multiplot.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3772.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1210,2590){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(1210,2738){\makebox(0,0)[r]{\strut{}$20000$}}%
      \put(1210,2886){\makebox(0,0)[r]{\strut{}$40000$}}%
      \put(1210,3034){\makebox(0,0)[r]{\strut{}$60000$}}%
      \put(1210,3181){\makebox(0,0)[r]{\strut{}$80000$}}%
      \put(1210,3329){\makebox(0,0)[r]{\strut{}$100000$}}%
      \put(1210,3477){\makebox(0,0)[r]{\strut{}$120000$}}%
      \put(1342,2370){\makebox(0,0){\strut{}$0$}}%
      \put(1814,2370){\makebox(0,0){\strut{}$100$}}%
      \put(2285,2370){\makebox(0,0){\strut{}$200$}}%
      \put(2757,2370){\makebox(0,0){\strut{}$300$}}%
      \put(3228,2370){\makebox(0,0){\strut{}$400$}}%
      \put(3700,2370){\makebox(0,0){\strut{}$500$}}%
      \put(4171,2370){\makebox(0,0){\strut{}$600$}}%
      \put(4643,2370){\makebox(0,0){\strut{}$700$}}%
      \put(3323,3455){\makebox(0,0){/:Bold Cluster Size 1}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,3070){\rotatebox{-270}{\makebox(0,0){\strut{}Kilobytes/Second}}}%
      \put(2992,2040){\makebox(0,0){\strut{}Runtime (Seconds)}}%
      \csname LTb\endcsname%%
      \put(3656,3378){\makebox(0,0)[r]{\strut{}No Containers}}%
      \csname LTb\endcsname%%
      \put(3656,3158){\makebox(0,0)[r]{\strut{}Docker}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1210,704){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(1210,852){\makebox(0,0)[r]{\strut{}$20000$}}%
      \put(1210,1000){\makebox(0,0)[r]{\strut{}$40000$}}%
      \put(1210,1148){\makebox(0,0)[r]{\strut{}$60000$}}%
      \put(1210,1296){\makebox(0,0)[r]{\strut{}$80000$}}%
      \put(1210,1444){\makebox(0,0)[r]{\strut{}$100000$}}%
      \put(1210,1592){\makebox(0,0)[r]{\strut{}$120000$}}%
      \put(1342,484){\makebox(0,0){\strut{}$0$}}%
      \put(1814,484){\makebox(0,0){\strut{}$100$}}%
      \put(2285,484){\makebox(0,0){\strut{}$200$}}%
      \put(2757,484){\makebox(0,0){\strut{}$300$}}%
      \put(3228,484){\makebox(0,0){\strut{}$400$}}%
      \put(3700,484){\makebox(0,0){\strut{}$500$}}%
      \put(4171,484){\makebox(0,0){\strut{}$600$}}%
      \put(4643,484){\makebox(0,0){\strut{}$700$}}%
      \put(3323,1570){\makebox(0,0){/:Bold Cluster Size 12}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,1185){\rotatebox{-270}{\makebox(0,0){\strut{}Kilobytes/Second}}}%
      \put(2992,154){\makebox(0,0){\strut{}Runtime (Seconds)}}%
      \csname LTb\endcsname%%
      \put(3656,1493){\makebox(0,0)[r]{\strut{}No Containers}}%
      \csname LTb\endcsname%%
      \put(3656,1273){\makebox(0,0)[r]{\strut{}Docker}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plots/storage_skylake/docker_network_usage_master_multiplot}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/storage_skylake/docker_nfs_symlinks_disk_usage_worker4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3772.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,704){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(946,1111){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(946,1517){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(946,1924){\makebox(0,0)[r]{\strut{}$600$}}%
      \put(946,2331){\makebox(0,0)[r]{\strut{}$800$}}%
      \put(946,2738){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(946,3144){\makebox(0,0)[r]{\strut{}$1200$}}%
      \put(946,3551){\makebox(0,0)[r]{\strut{}$1400$}}%
      \put(1078,484){\makebox(0,0){\strut{}$0$}}%
      \put(1672,484){\makebox(0,0){\strut{}$100$}}%
      \put(2266,484){\makebox(0,0){\strut{}$200$}}%
      \put(2861,484){\makebox(0,0){\strut{}$300$}}%
      \put(3455,484){\makebox(0,0){\strut{}$400$}}%
      \put(4049,484){\makebox(0,0){\strut{}$500$}}%
      \put(4643,484){\makebox(0,0){\strut{}$600$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,2127){\rotatebox{-270}{\makebox(0,0){\strut{}Milliseconds}}}%
      \put(2860,154){\makebox(0,0){\strut{}Runtime (Seconds)}}%
      \csname LTb\endcsname%%
      \put(3656,3378){\makebox(0,0)[r]{\strut{}Cluster Size 1}}%
      \csname LTb\endcsname%%
      \put(3656,3158){\makebox(0,0)[r]{\strut{}Cluster Size 12}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plots/storage_skylake/docker_nfs_symlinks_disk_usage_worker4}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/storage_skylake/docker_nfs_symlinks_disk_usage_worker4_multiplot.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3772.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,2590){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(946,2727){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(946,2865){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(946,3002){\makebox(0,0)[r]{\strut{}$600$}}%
      \put(946,3139){\makebox(0,0)[r]{\strut{}$800$}}%
      \put(946,3276){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(946,3414){\makebox(0,0)[r]{\strut{}$1200$}}%
      \put(946,3551){\makebox(0,0)[r]{\strut{}$1400$}}%
      \put(1078,2370){\makebox(0,0){\strut{}$0$}}%
      \put(1672,2370){\makebox(0,0){\strut{}$100$}}%
      \put(2266,2370){\makebox(0,0){\strut{}$200$}}%
      \put(2861,2370){\makebox(0,0){\strut{}$300$}}%
      \put(3455,2370){\makebox(0,0){\strut{}$400$}}%
      \put(4049,2370){\makebox(0,0){\strut{}$500$}}%
      \put(4643,2370){\makebox(0,0){\strut{}$600$}}%
      \put(2861,3455){\makebox(0,0){/:Bold Cluster Size 1}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,3070){\rotatebox{-270}{\makebox(0,0){\strut{}Milliseconds}}}%
      \put(2860,2040){\makebox(0,0){\strut{}Runtime (Seconds)}}%
      \csname LTb\endcsname%%
      \put(3656,3378){\makebox(0,0)[r]{\strut{}No Containers}}%
      \csname LTb\endcsname%%
      \put(3656,3158){\makebox(0,0)[r]{\strut{}Docker}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,704){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(946,841){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(946,979){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(946,1116){\makebox(0,0)[r]{\strut{}$600$}}%
      \put(946,1254){\makebox(0,0)[r]{\strut{}$800$}}%
      \put(946,1391){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(946,1529){\makebox(0,0)[r]{\strut{}$1200$}}%
      \put(946,1666){\makebox(0,0)[r]{\strut{}$1400$}}%
      \put(1078,484){\makebox(0,0){\strut{}$0$}}%
      \put(1672,484){\makebox(0,0){\strut{}$100$}}%
      \put(2266,484){\makebox(0,0){\strut{}$200$}}%
      \put(2861,484){\makebox(0,0){\strut{}$300$}}%
      \put(3455,484){\makebox(0,0){\strut{}$400$}}%
      \put(4049,484){\makebox(0,0){\strut{}$500$}}%
      \put(4643,484){\makebox(0,0){\strut{}$600$}}%
      \put(2861,1570){\makebox(0,0){/:Bold Cluster Size 12}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,1185){\rotatebox{-270}{\makebox(0,0){\strut{}Milliseconds}}}%
      \put(2860,154){\makebox(0,0){\strut{}Runtime (Seconds)}}%
      \csname LTb\endcsname%%
      \put(3656,1493){\makebox(0,0)[r]{\strut{}No Containers}}%
      \csname LTb\endcsname%%
      \put(3656,1273){\makebox(0,0)[r]{\strut{}Docker}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plots/storage_skylake/docker_nfs_symlinks_disk_usage_worker4_multiplot}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/storage_skylake/makespan_all_run_types.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3772.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,924){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(814,1299){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(814,1675){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(814,2050){\makebox(0,0)[r]{\strut{}$300$}}%
      \put(814,2425){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(814,2800){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(814,3176){\makebox(0,0)[r]{\strut{}$600$}}%
      \put(814,3551){\makebox(0,0)[r]{\strut{}$700$}}%
      \put(1364,704){\makebox(0,0){\strut{}no container}}%
      \put(1782,704){\makebox(0,0){\strut{}no container}}%
      \put(1782,484){\makebox(0,0){\strut{}nfs symlinks}}%
      \put(2200,704){\makebox(0,0){\strut{}docker}}%
      \put(2617,704){\makebox(0,0){\strut{}docker}}%
      \put(2617,484){\makebox(0,0){\strut{}nfs symlinks}}%
      \put(3035,704){\makebox(0,0){\strut{}singularity}}%
      \put(3453,704){\makebox(0,0){\strut{}singularity}}%
      \put(3453,484){\makebox(0,0){\strut{}nfs symlinks}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,2237){\rotatebox{-270}{\makebox(0,0){\strut{}Avg. Runtime (Seconds)}}}%
      \put(2408,154){\makebox(0,0){\strut{}Run Type}}%
      \csname LTb\endcsname%%
      \put(2884,3378){\makebox(0,0)[r]{\strut{}Cluster Size 1}}%
      \csname LTb\endcsname%%
      \put(2884,3158){\makebox(0,0)[r]{\strut{}Cluster Size 12}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plots/storage_skylake/makespan_all_run_types}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/storage_skylake/singularity_nfs_symlinks_disk_usage_worker4_multiplot.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3772.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,2590){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(946,2727){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(946,2865){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(946,3002){\makebox(0,0)[r]{\strut{}$600$}}%
      \put(946,3139){\makebox(0,0)[r]{\strut{}$800$}}%
      \put(946,3276){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(946,3414){\makebox(0,0)[r]{\strut{}$1200$}}%
      \put(946,3551){\makebox(0,0)[r]{\strut{}$1400$}}%
      \put(1078,2370){\makebox(0,0){\strut{}$0$}}%
      \put(1672,2370){\makebox(0,0){\strut{}$100$}}%
      \put(2266,2370){\makebox(0,0){\strut{}$200$}}%
      \put(2861,2370){\makebox(0,0){\strut{}$300$}}%
      \put(3455,2370){\makebox(0,0){\strut{}$400$}}%
      \put(4049,2370){\makebox(0,0){\strut{}$500$}}%
      \put(4643,2370){\makebox(0,0){\strut{}$600$}}%
      \put(2861,3455){\makebox(0,0){/:Bold Cluster Size 1}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,3070){\rotatebox{-270}{\makebox(0,0){\strut{}Milliseconds}}}%
      \put(2860,2040){\makebox(0,0){\strut{}Runtime (Seconds)}}%
      \csname LTb\endcsname%%
      \put(3656,3378){\makebox(0,0)[r]{\strut{}No Containers}}%
      \csname LTb\endcsname%%
      \put(3656,3158){\makebox(0,0)[r]{\strut{}Singularity}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,704){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(946,841){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(946,979){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(946,1116){\makebox(0,0)[r]{\strut{}$600$}}%
      \put(946,1254){\makebox(0,0)[r]{\strut{}$800$}}%
      \put(946,1391){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(946,1529){\makebox(0,0)[r]{\strut{}$1200$}}%
      \put(946,1666){\makebox(0,0)[r]{\strut{}$1400$}}%
      \put(1078,484){\makebox(0,0){\strut{}$0$}}%
      \put(1672,484){\makebox(0,0){\strut{}$100$}}%
      \put(2266,484){\makebox(0,0){\strut{}$200$}}%
      \put(2861,484){\makebox(0,0){\strut{}$300$}}%
      \put(3455,484){\makebox(0,0){\strut{}$400$}}%
      \put(4049,484){\makebox(0,0){\strut{}$500$}}%
      \put(4643,484){\makebox(0,0){\strut{}$600$}}%
      \put(2861,1570){\makebox(0,0){/:Bold Cluster Size 12}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,1185){\rotatebox{-270}{\makebox(0,0){\strut{}Milliseconds}}}%
      \put(2860,154){\makebox(0,0){\strut{}Runtime (Seconds)}}%
      \csname LTb\endcsname%%
      \put(3656,1493){\makebox(0,0)[r]{\strut{}No Containers}}%
      \csname LTb\endcsname%%
      \put(3656,1273){\makebox(0,0)[r]{\strut{}Singularity}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plots/storage_skylake/singularity_nfs_symlinks_disk_usage_worker4_multiplot}}%
    \gplfronttext
  \end{picture}%
\endgroup

